The "Colonial Impulse" of Natural Language Processing: An Audit of Bengali Sentiment Analysis Tools and Their Identity-based Biases

While colonization has sociohistorically impacted people's identities across various dimensions, those colonial values and biases continue to be perpetuated by sociotechnical systems. One category of sociotechnical systems--sentiment analysis tools--can also perpetuate colonial values and bias, yet less attention has been paid to how such tools may be complicit in perpetuating coloniality, although they are often used to guide various practices (e.g., content moderation). In this paper, we explore potential bias in sentiment analysis tools in the context of Bengali communities that have experienced and continue to experience the impacts of colonialism. Drawing on identity categories most impacted by colonialism amongst local Bengali communities, we focused our analytic attention on gender, religion, and nationality. We conducted an algorithmic audit of all sentiment analysis tools for Bengali, available on the Python package index (PyPI) and GitHub. Despite similar semantic content and structure, our analyses showed that in addition to inconsistencies in output from different tools, Bengali sentiment analysis tools exhibit bias between different identity categories and respond differently to different ways of identity expression. Connecting our findings with colonially shaped sociocultural structures of Bengali communities, we discuss the implications of downstream bias of sentiment analysis tools.

==> sections/all_tools.tex <==
\section{Curated BSA Tools and Their Inclusion/Exclusion}\label{app:all_tools}
\begin{table}[!ht]
    \centering
    \caption{PyPI packages (alphabetically sorted) identified using search phrases.}
    \label{tab:pypi_packages}
    \begin{tabular}{p{2cm}p{11cm}}
    \toprule
        \textbf{Package} & \textbf{Status and Rationale for Inclusion/Exclusion} \\
    \midrule
        BenDeep & The package supports sentiment analysis in Bengali and is operational. \inclusion{Therefore, we INCLUDED this package in our study.}\\\hline
        sbNLTK & We encountered a run-time error with the package. Despite reaching out to the developers, we received insufficient feedback to make it work. \exclusion{Hence, we did NOT include this tool in our study.}\\
    \bottomrule
    \end{tabular}
\end{table}

\begin{longtable}{p{3.5cm}p{9.5cm}}
    \caption{GitHub packages (alphabetically sorted) identified using search phrases. We reformatted underscores (snake\_cases) and CamelCases in repositories' names using spaces for better presentation.}
    \label{tab:github_packages}
    \\\hline
     \textbf{Package/Repository} & \textbf{Note on Reproducibility and Inclusion/Exclusion} \\
     \hline
     \endfirsthead
     \caption*{\textbf{Table \ref{tab:github_packages} continued:} GitHub packages identified using search phrases}
     \\\hline
     \textbf{Package/Repository} & \textbf{Note on Reproducibility and Inclusion/Exclusion} \\
     \hline
     \endhead % all the lines above this will be repeated on every page
     \hline
     \endfoot
    \hline
    abdulhasibuddin/Bangla-Sentiment-Analysis-with-GRU~\cite{alvi2022sentiment} & This repository provides source code and directs to the dataset developed by~\cite{tazim2018bengali} it used to train the model. However, the code encountered runtime errors despite several attempts to fix the code. \exclusion{That's why, we did NOT include this repository in our study.} \\\hline
    Amxadhussain97/Bangla-Sentiment-Analysis-on-Covid-19-Texts-NLP-~\cite{tamim2021bangla} & This repository includes source codes. However, they did not include the trained models or any of the training and testing data they referred to from within the codes. Moreover, from the cached output, the repository seems to be one for emotion classification. Though related, it is out of the scope of our study on Bengali sentiment analysis. \exclusion{Therefore, we decided NOT to include this in our study.}\\\hline
    anwar-arif/SentimentAnalysis~\cite{arif2018sentiment} & This repository includes source codes but does not include any of the training and testing data they referred to from within the codes, nor a trained model. \exclusion{Hence, we decided NOT to include this in our study.}\\\hline
    Ayubur/bangla-sentiment-analysis-chatbot~\cite{rahman2020bangla} & Though this repository does not provide the source codes used to do sentiment analysis, it includes the trained BSA model. We can use that for BSA tasks without the chatbot front end. However, the trained model's pipeline was not configured to predict corresponding probabilities with binary classes. \exclusion{Hence, we decided NOT to include the model as a tool in our study.}\\\hline
    Ayubur/bangla-sentiment-analysis-datasets~\cite{rahman2019bangla} & This repository does not contain source codes or models for sentiment analysis, but datasets. \exclusion{Therefore, we did NOT include this repository in our study.}\\\hline %The previous repository~\cite{rahman2020bangla} was also developed by the same GitHub user.
    dgted/bengaliNLP~\cite{alam2019bengaliNLP} & The source codes were sufficient to recreate the tool. \inclusion{We INCLUDED this tool in our study.}\\\hline
    DhrubaDC1/Bengali-Sentiment-Analysis~\cite{chakraborty2023bengali} & The source code and dataset were sufficient to recreate the models with modifications for binary prediction. \inclusion{We have INCLUDED this repository in our study.}\\\hline
    eshadutta/NLP Bengali Sentiment Analysis~\cite{dutta2021nlp} & The source codes and datasets were sufficient to recreate the models. \inclusion{We have INCLUDED this repository in our study.}\\\hline
    HimelMazumder/machine-learning-in-bangla-sentiment-analysis~\cite{mazumder2023machine} & The source could not be used to generate a model and calculate sentiment scores for sample test sentences. \exclusion{Hence, we did NOT include this repository in our study.}\\\hline
    Imran-cse/Bengali-Sentiment-Analysis~\cite{hossain2018bengali} & This repository only contains a few lexicon dictionaries. There are no trained models or source codes available. \exclusion{Hence, we decided NOT to include this repository in our analysis.}\\\hline
    kishormorol/BSA~\cite{morol2021bsa} & This repository includes only a README file, but no source codes and models. \exclusion{Hence, we did NOT include this repository in our study.}\\\hline
    Mahdi-Abdullah/Bangla-Sentiment-Analysis~\cite{mahdi2023sentiment} & The repository was well-organized with source code, data, and trained model. \inclusion{We INCLUDED this repository in our study.}\\\hline
    mhtarek/Bangla-sentiment-analysis-by-using-RNN~\cite{tarek2019bangla} & The source codes and datasets were sufficient to recreate the models with modifications for binary prediction. \inclusion{We have INCLUDED this repository in our study.}\\\hline
    mubina8/Bengali sentiment analysis~\cite{ashrafi2022bengali} & This is an empty repository. \exclusion{Hence, we did NOT include this repository in our study.}\\\hline
    nafistiham/Academic-Thesis~\cite{tiham2019academict} & The repository provided a trained Bengali sentiment analysis model. \inclusion{We have INCLUDED the BiLSTM model from this repository in our study.}\\\hline
    Neloy262/Bangla-Sentiment-Analysis~\cite{neloy2022bangla} & The repository contains source codes and data to produce the trained model. \inclusion{We have INCLUDED this repository in our study.}\\\hline
    NitishOritro/BanglaSentimentAnalysis~\cite{bhowmik2021bangla} & The repository includes only a tokenizer, a stemmer, and a POS tagger but does not include the latter modules described in the paper. Since we could not replicate the complete sentiment analysis tool from the partial codes, \exclusion{we did NOT include the repository in our study.}\\\hline
    NuhashHaque/Bangla-Sentiment-Analysis-with-CNN-BiLSTM-based-Hybrid-Network~\cite{haque2020bangla} & The source codes and datasets were sufficient to recreate the models. \inclusion{We have INCLUDED this repository in our study.}\\\hline
    omarfarabi/Bengali sentiment analysis~\cite{farabi2020bengali} & This repository contains the same source codes and dataset as mhtarek/Bangla-sentiment-analysis-by-using-RNN~\cite{tarek2019bangla} which we have already included. \exclusion{Therefore, to avoid repetition, we have NOT included this repository in our study.}\\\hline
    rabiul-ju/BanglaSentimentAnalysis~\cite{alam2017bangla} & The source codes and datasets were for emotion prediction task, not sentiment analysis. \exclusion{Since this is out of scope, we did NOT include this repository in our study.}\\\hline
    rizveeredwan/bn-sentiment-analysis~\cite{rizvee2022bn} & From matching the filenames in the dataset directory with the Jupyter Notebook checkpoints, it seems that the datasets included in the repository are not the ones referred to from within the source codes. Because of this discrepancy, we could not replicate the original tool. \exclusion{Therefore, we did NOT include this repository in our study.}\\\hline
    Rumaisa10/Bangla Sentiment analysis~\cite{rumaisa2023bangla} & This repository includes source codes but does not include any of the training and testing data they referred to from within the codes, nor a trained model. \exclusion{Hence, we decided NOT to include this in our study.}\\\hline
    SamantaRuhee/Bangla-Sentiment-Analysis~\cite{ruhee2021bangla} & The source codes and datasets were sufficient to recreate the models with modifications for binary prediction. \inclusion{We have INCLUDED this repository in our study.}\\\hline
    Sanzidikawsar/Bangla-Sentiment-Analysis~\cite{kawsar2017bangla} & The code in this repository basically translates Bengali sentences to English and uses TextBlob's sentiment analysis function to predict polarities of Bengali sentences. source codes are sufficient to replicate the tool. Since (1) bias in English sentiment analysis tools are well-studied and (2) the Google translate API used in this repository has a daily usage limit, making it impractical for the large-scale audit in our study. \exclusion{Therefore, we did NOT include this repository in our study.}\\\hline
    shahriarshakil0/Bangla Sentiment Analysis~\cite{hassan2022sentiment} & The repository provided the trained models. \inclusion{We INCLUDED this repository as a tool in our study.}\\\hline
    shahrukhx01/nnti hindi bengali sentiment analysis~\cite{khan2022sentiment} & The trained models provided in the repository are for a hate speech classifier. Though related, it is out of the scope of our study on Bengali sentiment analysis tools. \exclusion{That's why we did NOT include this repository in our study.}\\\hline
    ShaikaChowdhury/Bangla Sentiment Analysis~\cite{chowdhury2020bangla} & This repository does not include source codes or models, but a dataset used in a paper~\cite{chowdhury2014performing}. \exclusion{Consequently, we did NOT consider this repository as a BSA tool in our study.}\\\hline
    SouvikHalder32/Bengali Sentiment Analysis~\cite{halder2023bengali} & This is an empty repository. \exclusion{Hence, we did NOT include this repository in our study.}\\\hline
    tanzid2059/Bangla-Sentiment-Analysis-using-semi-supervise-learning-model~\cite{ferdoush2021bangla} & This repository includes source codes, but it does not include the authors' labeled data necessary for this semi-supervised model. We also did not have access to a model trained on their labeled data. \exclusion{Hence, we decided NOT to include this in our study.}\\\hline
    Tariq-amir/Bangla-Sentiment-Analysis~\cite{amir2023bangla} & The information in this repository was sufficient to replicate the result. \inclusion{Hence, we could INCLUDE this tool in our study.}\\\hline
    yeamin21/Bengali-Sentiment-Analysis~\cite{mahmud2021bengali} & The source codes and datasets~\cite{sazzed2020cross} were sufficient to recreate the models with modifications for binary prediction. \inclusion{We have INCLUDED this repository in our study.}\\\hline
\end{longtable}

==> sections/app_rq2.1.tex <==
\section{Matrices of BSA tools' direction of bias and their developers' demographic backgrounds}

\begin{table}[!ht]
    \centering
    \begin{tabular}{c|p{1cm}|p{1cm}|p{1cm}}
        \hline
        \diagbox[width=2.5cm]{bias}{developer} &  female & male & female+ male \\\hline
        female & T10 &  T9, T12, T13 & T11 \\\hline
        male  & - &  T2, T5, T7 & - \\\hline
        no & - & T1, T3, T6 & T4 \\\hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|p{1cm}|p{1cm}}
        \hline
        \diagbox[width=2.5cm]{bias}{developer} &  Hindu & Muslim  \\\hline
        Hindu & T1, T4 & T10, T13 \\\hline
        Muslim & T3 & T6, T7, T9 \\\hline
        no & - & T2, T5, T11, T12 \\\hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\begin{table}[]
    \centering
    \begin{tabular}{c|p{1.7cm}|p{1cm}}
        \hline
        \diagbox[width=2.5cm]{bias}{developer} &  Bangladeshi & Indian  \\\hline
        Bangladeshi & T1-T3, T5-T7, T11-T13 & T4 \\\hline
        Indian  & 9 & - \\\hline
        no & 10 & - \\\hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

==> sections/hypothesis_test_results.tex <==
\section{Results of Hypothesis Tests}

\subsection{Details about tests in RQ1}\label{app:rq1}

\begin{table}[!ht]
    \centering
    \caption{Results of Kruskal-Wallis analysis of variance of different sentiment analysis tools' mean scores for (a) female, (b) male, (c) Hindu, (d) Muslim, (e) Bangladeshi, and (e) Indian identity categories. Here, the larger the H-statistic values are, the stronger the evidence against the null hypotheses.}
    \label{tab:rq1}
    \begin{tabular}{p{1.7cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.85cm}|p{1.5cm}}
    \hline
                    & \textbf{Female} & \textbf{Male} & \textbf{Hindu} & \textbf{Muslim} & \textbf{Bangladeshi} & \textbf{Indian} \\\hline
        \textbf{H-statistic} & 5.79e+04 & 7.30e+04 & 3.66e+04 & 3.85e+04 & 6.57e+04 & 6.33e+04 \\\hline
        \textbf{p-value}     & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 & 0.0000 \\\hline
        \textbf{Power}       & \textbf{1.0} & \textbf{1.0} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\\hline
    \end{tabular}
\end{table}

% While most pairwise comparisons between BSA tools showed significantly different sentiment scores for a fixed identity category, the pairs that did not show significant differences in their sentiment scores are listed below (values in parentheses show the corresponding p-values\footnote{Significance at 0.0001, 0.001, and 0.01 are indicated by ***, **, and *, respectively.}):

% \begin{itemize}
%     \item Female: T6-T10 {\footnotesize(0.7)}
%     \item Male: T8-T10 {\footnotesize(6e-3*)}
%     \item Hindu: T3-T6 {\footnotesize(2e-3*)}
%     \item Muslim: T1-T5 {\footnotesize(0.1)}, T1-T13 {\footnotesize(0.7)}, T2-T4 {\footnotesize(8e-3*)}, T3-T10 {\footnotesize(0.8)}, T5-T9 {\footnotesize(2e-4**)}, T5-13 {\footnotesize(0.7)}, T6-T8 {\footnotesize(0.08)}, T7-T12 {\footnotesize(0.01)}
%     \item Bangladeshi: T4-T12 {\footnotesize(0.05)}, T5-T9 {\footnotesize(7e-5***)}, T7-T12 {\footnotesize(5e-5***)}, T8-10 {\footnotesize(0.7)}
%     \item Indian: T2-T8 {\footnotesize(0.3)}, T3-T10 {\footnotesize(0.9)}
% \end{itemize}

The following Tables present the detailed results from posthoc tests:


% \begin{landscape}
{\tiny

\begin{table}[!ht]
\caption{Conover-Iman test across BSA tool pairs for Female identity category}
\label{tab:conover_female}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
 & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{T7} & \textbf{T8} & \textbf{T9} & \textbf{T10} & \textbf{T11} & \textbf{T12} & \textbf{T13} \\
\midrule
\textbf{T1} & 1.0 \\
\textbf{T2} & 0.0 & 1.0 \\
\textbf{T3} & 0.0 & 1e-23 & 1.0 \\
\textbf{T4} & 0.0 & 1e-253 & 0.0 & 1.0 \\
\textbf{T5} & 2e-39 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T6} & 0.0 & 3e-50 & 3e-06 & 0.0 & 0.0 & 1.0 \\
\textbf{T7} & 0.0 & 1e-42 & 1e-126 & 3e-90 & 0.0 & 1e-182 & 1.0 \\
\textbf{T8} & 2e-88 & 0.0 & 0.0 & 0.0 & 3e-242 & 0.0 & 0.0 & 1.0 \\
\textbf{T9} & 4e-30 & 0.0 & 0.0 & 0.0 & 4e-135 & 0.0 & 0.0 & 1e-16 & 1.0 \\
\textbf{T10} & 0.0 & 1e-47 & 2e-05 & 0.0 & 0.0 & 7e-01 & 1e-177 & 0.0 & 0.0 & 1.0 \\
\textbf{T11} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T12} & 0.0 & 2e-85 & 2e-195 & 5e-46 & 0.0 & 1e-263 & 2e-08 & 0.0 & 0.0 & 1e-257 & 0.0 & 1.0 \\
\textbf{T13} & 5e-165 & 0.0 & 0.0 & 0.0 & 0.0 & 3e-289 & 0.0 & 5e-13 & 6e-56 & 1e-295 & 0.0 & 0.0 & 1.0 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{Conover-Iman test across BSA tool pairs for Male identity category}
\label{tab:conover_male}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
 & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{T7} & \textbf{T8} & \textbf{T9} & \textbf{T10} & \textbf{T11} & \textbf{T12} & \textbf{T13} \\
\midrule
\textbf{T1} & 1.0 \\
\textbf{T2} & 0.0 & 1.0 \\
\textbf{T3} & 0.0 & 2e-192 & 1.0 \\
\textbf{T4} & 0.0 & 6e-206 & 0.0 & 1.0 \\
\textbf{T5} & 3e-17 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T6} & 0.0 & 1e-72 & 7e-30 & 0.0 & 0.0 & 1.0 \\
\textbf{T7} & 0.0 & 1e-106 & 0.0 & 2e-17 & 0.0 & 0.0 & 1.0 \\
\textbf{T8} & 0.0 & 5e-303 & 8e-14 & 0.0 & 0.0 & 1e-80 & 0.0 & 1.0 \\
\textbf{T9} & 5e-76 & 0.0 & 0.0 & 0.0 & 1e-22 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T10} & 0.0 & 2e-260 & 2e-06 & 0.0 & 0.0 & 1e-59 & 0.0 & 6e-03 & 0.0 & 1.0 \\
\textbf{T11} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0  \\
\textbf{T12} & 0.0 & 2e-25 & 0.0 & 4e-89 & 0.0 & 2e-180 & 1e-29 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T13} & 2e-78 & 0.0 & 0.0 & 0.0 & 3e-165 & 0.0 & 0.0 & 5e-228 & 1e-305 & 7e-268 & 0.0 & 0.0 & 1.0 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{Conover-Iman test across BSA tool pairs for Hindu identity category}
\label{tab:conover_hindu}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
 & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{T7} & \textbf{T8} & \textbf{T9} & \textbf{T10} & \textbf{T11} & \textbf{T12} & \textbf{T13} \\
\midrule
\textbf{T1} & 1.0 \\
\textbf{T2} & 0.0 & 1.0 \\
\textbf{T3} & 3e-266 & 5e-281 & 1.0 \\
\textbf{T4} & 0.0 & 8e-55 & 0.0 & 1.0 \\
\textbf{T5} & 3e-07 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T6} & 0.0 & 6e-235 & 2e-03 & 0.0 & 0.0 & 1.0 \\
\textbf{T7} & 5e-193 & 0.0 & 7e-07 & 0.0 & 7e-269 & 5e-16 & 1.0 \\
\textbf{T8} & 0.0 & 3e-64 & 2e-78 & 2e-234 & 0.0 & 4e-55 & 3e-127 & 1.0 \\
\textbf{T9} & 2e-169 & 0.0 & 0.0 & 0.0 & 2e-110 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T10} & 0.0 & 5e-106 & 2e-43 & 0.0 & 0.0 & 1e-26 & 6e-81 & 2e-06 & 0.0 & 1.0 \\
\textbf{T11} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T12} & 0.0 & 5e-25 & 0.0 & 7e-07 & 0.0 & 0.0 & 0.0 & 3e-166 & 0.0 & 3e-230 & 0.0 & 1.0 \\
\textbf{T13} & 8e-23 & 0.0 & 3e-136 & 0.0 & 1e-52 & 7e-172 & 1e-85 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{Conover-Iman test across BSA tool pairs for Muslim identity category}
\label{tab:conover_muslim}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
 & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{T7} & \textbf{T8} & \textbf{T9} & \textbf{T10} & \textbf{T11} & \textbf{T12} & \textbf{T13} \\
\midrule
\textbf{T1} & 1.0 \\
\textbf{T2} & 0.0 & 1.0 \\
\textbf{T3} & 0.0 & 8e-191 & 1.0 \\
\textbf{T4} & 0.0 & 8e-03 & 1e-151 & 1.0 \\
\textbf{T5} & 1e-01 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T6} & 0.0 & 9e-105 & 2e-13 & 3e-76 & 0.0 & 1.0 \\
\textbf{T7} & 0.0 & 8e-19 & 0.0 & 6e-34 & 0.0 & 2e-209 & 1.0 \\
\textbf{T8} & 0.0 & 4e-83 & 7e-23 & 5e-58 & 0.0 & 8e-02 & 2e-178 & 1.0 \\
\textbf{T9} & 2e-09 & 0.0 & 0.0 & 0.0 & 2e-04 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T10} & 0.0 & 8e-187 & 8e-01 & 4e-148 & 0.0 & 2e-12 & 0.0 & 1e-21 & 0.0 & 1.0 \\
\textbf{T11} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T12} & 0.0 & 1e-08 & 1e-276 & 2e-19 & 0.0 & 2e-170 & 1e-02 & 2e-142 & 0.0 & 9e-272 & 0.0 & 1.0 \\
\textbf{T13} & 7e-01 & 0.0 & 0.0 & 0.0 & 7e-01 & 0.0 & 0.0 & 0.0 & 2e-06 & 0.0 & 0.0 & 0.0 & 1.0 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{Conover-Iman test across BSA tool pairs for Bangladeshi identity category}
\label{tab:conover_bangladeshi}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
 & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{T7} & \textbf{T8} & \textbf{T9} & \textbf{T10} & \textbf{T11} & \textbf{T12} & \textbf{T13} \\
\midrule
\textbf{T1} & 1.0 \\
\textbf{T2} & 0.0 & 1.0 \\
\textbf{T3} & 0.0 & 0.0 & 1.0 \\
\textbf{T4} & 0.0 & 2e-247 & 3e-12 & 1.0 \\
\textbf{T5} & 2e-30 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T6} & 0.0 & 3e-59 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T7} & 0.0 & 3e-160 & 2e-42 & 2e-10 & 0.0 & 0.0 & 1.0 \\
\textbf{T8} & 0.0 & 3e-124 & 0.0 & 0.0 & 0.0 & 8e-13 & 0.0 & 1.0 \\
\textbf{T9} & 8e-13 & 0.0 & 0.0 & 0.0 & 7e-05 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T10} & 0.0 & 2e-128 & 0.0 & 0.0 & 0.0 & 4e-14 & 0.0 & 7e-01 & 0.0 & 1.0 \\
\textbf{T11} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T12} & 0.0 & 8e-216 & 3e-20 & 5e-02 & 0.0 & 0.0 & 5e-05 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T13} & 6e-53 & 0.0 & 0.0 & 0.0 & 5e-161 & 0.0 & 0.0 & 7e-288 & 4e-115 & 1e-281 & 0.0 & 0.0 & 1.0 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[!ht]
\caption{Conover-Iman test across BSA tool pairs for Indian identity category}
\label{tab:conover_indian}
\begin{tabular}{lrrrrrrrrrrrrr}
\toprule
 & \textbf{T1} & \textbf{T2} & \textbf{T3} & \textbf{T4} & \textbf{T5} & \textbf{T6} & \textbf{T7} & \textbf{T8} & \textbf{T9} & \textbf{T10} & \textbf{T11} & \textbf{T12} & \textbf{T13} \\
\midrule
\textbf{T1} & 1.0 \\
\textbf{T2} & 0.0 & 1.0 \\
\textbf{T3} & 0.0 & 7e-107 & 1.0 \\
\textbf{T4} & 0.0 & 3e-181 & 0.0 & 1.0 \\
\textbf{T5} & 4e-22 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T6} & 0.0 & 6e-64 & 1e-06 & 0.0 & 0.0 & 1.0 \\
\textbf{T7} & 0.0 & 8e-09 & 2e-172 & 1e-113 & 0.0 & 3e-116 & 1.0 \\
\textbf{T8} & 0.0 & 3e-01 & 3e-94 & 1e-198 & 0.0 & 3e-54 & 8e-13 & 1.0 \\
\textbf{T9} & 0.0 & 0.0 & 1e-146 & 0.0 & 0.0 & 4e-209 & 0.0 & 0.0 & 1.0 \\
\textbf{T10} & 0.0 & 8e-108 & 9e-01 & 0.0 & 0.0 & 9e-07 & 9e-174 & 3e-95 & 2e-145 & 1.0 \\
\textbf{T11} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T12} & 0.0 & 5e-84 & 0.0 & 1e-19 & 0.0 & 7e-291 & 1e-40 & 6e-96 & 0.0 & 0.0 & 0.0 & 1.0 \\
\textbf{T13} & 1e-211 & 0.0 & 0.0 & 0.0 & 3e-99 & 0.0 & 0.0 & 0.0 & 2e-97 & 0.0 & 0.0 & 0.0 & 1.0 \\
\bottomrule
\end{tabular}
\end{table}

}% \end{landscape}

\clearpage
\subsection{Details about hypothesis tests in RQ2}\label{app:rq2}

% \subsubsection{Gender}
\begin{longtable}{p{1cm}|p{4cm}|p{4cm}|p{4cm}}
    \caption{Results of Wilcoxon signed-rank test between female and male gender-based identities in each examined Bengali sentiment analysis tool, with null hypothesis $(\mu_{female}=\mu_{male})$ and alternative hypotheses in different directions}
    \label{tab:rq2_gender}
    \\\hline
     \textbf{Tool} & \textbf{$\mu_{female}\neq\mu_{male}$} & \textbf{$\mu_{female}<\mu_{male}$} & \textbf{$\mu_{female}>\mu_{male}$} \\
     \hline
     \endfirsthead
     \caption*{\textbf{Table \ref{tab:rq2_gender} continued:} Wilcoxon signed-rank test for female and male gender-based identities}
     \\\hline
     \textbf{Tool} & \textbf{$\mu_{female}\neq\mu_{male}$} & \textbf{$\mu_{female}<\mu_{male}$} & \textbf{$\mu_{female}>\mu_{male}$} \\
     \hline
     \endhead % all the lines above this will be repeated on every page
     \hline
     \endfoot
    \hline
    \textcolor{black}{\textbf{T1}} & W-statistic: 1.57e+08 \newline p-value: 1.10e-07*** \newline Power: 0.2 & W-statistic: 1.57e+08 \newline p-value: 5.48e-08*** \newline Power: 0.2 & W-statistic: 1.57e+08 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T2} & W-statistic: 7.30e+07 \newline p-value: 7.55e-180*** \newline Power: \textbf{1.0} & W-statistic: 7.30e+07 \newline p-value: 3.78e-180*** \newline Power: \textbf{1.0} & W-statistic: 7.30e+07 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textcolor{black}{\textbf{T3}} & W-statistic: 7.19e+07 \newline p-value: 1.47e-12*** \newline Power: 0.2 & W-statistic: 8.14e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 8.14e+07 \newline p-value: 7.33e-13*** \newline Power: 0.2 \\\hline
    \textcolor{black}{\textbf{T4}} & W-statistic: 5.26e+07 \newline p-value: 1.16e-13*** \newline Power: 0.1 & W-statistic: 6.05e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 6.05e+07 \newline p-value: 5.80e-14*** \newline Power: 0.2 \\\hline
    \textbf{T5} & W-statistic: 9.37e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 9.37e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 9.37e+06 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textcolor{black}{\textbf{T6}} & W-statistic: 0.0 \newline p-value: 0.317 \newline Power: 0.0 & W-statistic: 0.0 \newline p-value: 0.159 \newline Power: 0.0 & W-statistic: 0.0 \newline p-value: 0.841 \newline Power: 0.0 \\\hline
    \textbf{T7} & W-statistic: 6.93e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 6.93e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 6.93e+07 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T8} & W-statistic: 8.47e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 8.47e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 8.47e+07 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T9} & W-statistic: 2.51e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 1.84e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.84e+08 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T10} & W-statistic: 7.58e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 1.35e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.35e+08 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T11} & W-statistic: 1.78e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 1.11e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.11e+08 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T12} & W-statistic: 4.97e+07 \newline p-value: 2.67e-283*** \newline Power: \textbf{1.0} & W-statistic: 9.60e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 9.60e+07 \newline p-value: 1.33e-283*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T13} & W-statistic: 9.14e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 1.68e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.68e+08 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
\end{longtable}

% \subsubsection{Religion}
\begin{longtable}{p{1cm}|p{4cm}|p{4cm}|p{4cm}}
    \caption{Results of Wilcoxon signed-rank test between Hindu and Muslim religion-based identities in each examined Bengali sentiment analysis tool, with null hypothesis $(\mu_{Hindu}=\mu_{Muslim})$ and alternative hypotheses ($H_{RA}$) in different directions}
    \label{tab:rq2_religion}
    \\\hline
     \textbf{Tool} & \textbf{$\mu_{Hindu}\neq\mu_{Muslim}$} & \textbf{$\mu_{Hindu}<\mu_{Muslim}$} & \textbf{$\mu_{Hindu}>\mu_{Muslim}$} \\
     \hline
     \endfirsthead
     \caption*{\textbf{Table \ref{tab:rq2_religion} continued:} Wilcoxon signed-rank test for Hindu and Muslim religion-based identities}
     \\\hline
     \textbf{Tool} & \textbf{$\mu_{Hindu}\neq\mu_{Muslim}$} & \textbf{$\mu_{Hindu}<\mu_{Muslim}$} & \textbf{$\mu_{Hindu}>\mu_{Muslim}$} \\
     \hline
     \endhead % all the lines above this will be repeated on every page
     \hline
     \endfoot
    \hline
    \textbf{T1} & W-statistic: 3.15e+07 \newline p-value: 1.89e-30*** \newline Power: \textbf{0.8} & W-statistic: 4.02e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 4.02e+07 \newline p-value: 9.46e-31*** \newline Power: \textbf{0.9} \\\hline
    \textcolor{black}{\textbf{T2}} & W-statistic: 3.34e+07 \newline p-value: 1.11e-12*** \newline Power: 0.2 & W-statistic: 3.34e+07 \newline p-value: 5.57e-13*** \newline Power: 0.3 & W-statistic: 3.34e+07 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T3} & W-statistic: 4.13e+03 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 4.13e+03 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 4.13e+03 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T4} & W-statistic: 9.56e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 5.03e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 5.03e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textcolor{black}{\textbf{T5}} & W-statistic: 2.91e+07 \newline p-value: 0.779 \newline Power: 0.0 & W-statistic: 2.93e+07 \newline p-value: 0.611 \newline Power: 0.0 & W-statistic: 2.93e+07 \newline p-value: 0.389 \newline Power: 0.0 \\\hline
    \textbf{T6} & W-statistic: 0.0 \newline p-value: 1.02e-277*** \newline Power: \textbf{1.0} & W-statistic: 0.0 \newline p-value: 5.08e-278*** \newline Power: \textbf{1.0} & W-statistic: 0.0 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T7} & W-statistic: 3.62e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 3.62e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 3.62e+06 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T8} & W-statistic: 3.00e+07 \newline p-value: 3.82e-57*** \newline Power: \textbf{1.0} & W-statistic: 3.00e+07 \newline p-value: 1.91e-57*** \newline Power: \textbf{1.0} & W-statistic: 3.00e+07 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T9} & W-statistic: 9.87e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 9.87e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 9.87e+06 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T10} & W-statistic: 8.33e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 6.39e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 6.39e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textcolor{black}{\textbf{T11}} & W-statistic: 0.0 \newline p-value: 0.317 \newline Power: 0.0 & W-statistic: 1.0 \newline p-value: 0.841 \newline Power: 0.0 & W-statistic: 1.0 \newline p-value: 0.159 \newline Power: 0.0 \\\hline
    \textcolor{black}{\textbf{T12}} & W-statistic: 1.49e+07 \newline p-value: 3.76e-17*** \newline Power: 0.3 & W-statistic: 1.85e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.85e+07 \newline p-value: 1.88e-17*** \newline Power: 0.4 \\\hline
    \textbf{T13} & W-statistic: 8.86e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 6.34e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 6.34e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
\end{longtable}

% \subsubsection{Nationality}
\begin{longtable}{p{1cm}|p{4cm}|p{4cm}|p{4cm}}
    \caption{Results of Wilcoxon signed-rank test between Bangladeshi and Indian nationality-based identities in each examined Bengali sentiment analysis tool, with null hypothesis $(\mu_{Bangladeshi}=\mu_{Indian})$ and alternative hypotheses ($H_{NA}$) in different directions}
    \label{tab:rq2_nationality}
    \\\hline
     \textbf{Tool} & \textbf{$\mu_{Bangladeshi}\neq\mu_{Indian}$} & \textbf{$\mu_{Bangladeshi}<\mu_{Indian}$} & \textbf{$\mu_{Bangladeshi}>\mu_{Indian}$} \\
     \hline
     \endfirsthead
     \caption*{\textbf{Table \ref{tab:rq2_nationality} continued:} Wilcoxon signed-rank test for Bangladeshi and Indian nationality-based identities}
     \\\hline
     \textbf{Tool} & \textbf{$\mu_{Bangladeshi}\neq\mu_{Indian}$} & \textbf{$\mu_{Bangladeshi}<\mu_{Indian}$} & \textbf{$\mu_{Bangladeshi}>\mu_{Indian}$} \\
     \hline
     \endhead % all the lines above this will be repeated on every page
     \hline
     \endfoot
    \hline
    \textbf{T1} & W-statistic: 7.50e+07 \newline p-value: 1.03e-247*** \newline Power: \textbf{1.0} & W-statistic: 1.31e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.31e+08 \newline p-value: 5.13e-248*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T2} & W-statistic: 7.73e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 2.42e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 2.42e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T3} & W-statistic: 2.56e+05 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 1.35e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.35e+08 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T4} & W-statistic: 5.73e+07 \newline p-value: 1.74e-134*** \newline Power: \textbf{1.0} & W-statistic: 8.92e+07 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 8.92e+07 \newline p-value: 8.70e-135*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T5} & W-statistic: 5.78e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 1.31e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.31e+08 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T6} & W-statistic: 0.00.0 \newline p-value: 1.09e-51*** \newline Power: \textbf{1.0} & W-statistic: 2.94e+04 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 2.94e+04 \newline p-value: 5.43e-52*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T7} & W-statistic: 7.51e+07 \newline p-value: 9.34e-156*** \newline Power: \textbf{1.0} & W-statistic: 1.17e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.17e+08 \newline p-value: 4.67e-156*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T8} & W-statistic: 5.74e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 5.74e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 5.74e+07 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T9} & W-statistic: 2.29e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 2.29e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 2.29e+07 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textcolor{black}{\textbf{T10}} & W-statistic: 9.32e+07 \newline p-value: 1.54e-15*** \newline Power: 0.2 & W-statistic: 9.32e+07 \newline p-value: 7.70e-16*** \newline Power: 0.3 & W-statistic: 9.32e+07 \newline p-value: 1.0 \newline Power: 0.0 \\\hline
    \textbf{T11} & W-statistic: 4.76e+05 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 8.92e+06 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 8.92e+06 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T12} & W-statistic: 4.10e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 1.02e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.02e+08 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
    \textbf{T13} & W-statistic: 6.03e+07 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} & W-statistic: 1.39e+08 \newline p-value: 1.0 \newline Power: 0.0 & W-statistic: 1.39e+08 \newline p-value: 0.0000*** \newline Power: \textbf{1.0} \\\hline
\end{longtable}



